Engineering LaCAM$^\ast$: Towards Real-Time, Large-Scale, and Near-Optimal Multi-Agent Pathfinding

This paper addresses the challenges of real-time, large-scale, and near-optimal multi-agent pathfinding (MAPF) through enhancements to the recently proposed LaCAM* algorithm. LaCAM* is a scalable search-based algorithm that guarantees the eventual finding of optimal solutions for cumulative transition costs. While it has demonstrated remarkable planning success rates, surpassing various state-of-the-art MAPF methods, its initial solution quality is far from optimal, and its convergence speed to the optimum is slow. To overcome these limitations, this paper introduces several improvement techniques, partly drawing inspiration from other MAPF methods. We provide empirical evidence that the fusion of these techniques significantly improves the solution quality of LaCAM*, thus further pushing the boundaries of MAPF algorithms.

==> algo/pibt.tex <==
{
  %
  \begin{algorithm}[th!]
    \caption{PIBT}
    \label{algo:pibt}
    %
    \begin{algorithmic}[1]
      \Input{configuration $\Q\from$, agents $A$, goals \G}
      \Output{configuration $\Q\to$ (each element is initialized with $\bot$)}
      %
      \State \textbf{for}~$i \in A$~\textbf{do};~
             \textbf{if}~{$\Q\to[i] = \bot$}~\textbf{then}~{$\PIBT(i)$}
      \label{algo:pibt:call-func}
      \State \Return $\Q\to$
      \label{algo:pibt:top:end}
      %
      \Procedure{\PIBT}{$i$}
      \Comment{return \valid or \invalid}
      \label{algo:pibt:recursive:start}
      \State $C \leftarrow \neigh(\Q\from[i]) \cup \left\{\Q\from[i]\right\}$
      \label{algo:pibt:cand}
      \Comment{candidate vertices}
      \State sort $C$ in ascending order of $\dist(u, g_i)$ where $u \in C$
      \label{algo:pibt:sort}
      %
      \For{$v \in C$}
      \label{algo:pibt:loop-start}
      %
      \IfSingle{collisions in $\Q\to$ supposing $\Q\to[i]=v$}{\Continue}
      \label{algo:pibt:collision-check}
      %
      \State $\Q\to[i] \leftarrow v$
      \label{algo:pibt:reserve}
      %
      \If{$\exists j \in A~\text{s.t.}~j \neq i \land \Q\from[j]=v \land \Q\to[j]=\bot$}
      \label{algo:pibt:check-k}
      %
      \IfSingle{$\PIBT(j)= \invalid$}{\Continue}
      \label{algo:pibt:call-pi}
      \EndIf
      \State \Return~\valid
      \Comment{assignment done}
      \label{algo:pibt:valid}
      %
      \EndFor
      \label{algo:pibt:loop-end}
      %
      \State $\Q\to[i] \leftarrow \Q\from[i]$;~\Return~\invalid
      \label{algo:pibt:stay}
      %
      \EndProcedure
      \label{algo:pibt:recursive:end}
    \end{algorithmic}
  \end{algorithm}
}


==> fig/maps.tex <==
{
  \setlength{\tabcolsep}{2pt}
  \newcommand{\figcol}[3]{
    \begin{minipage}{0.32\linewidth}
      \centering
      {\mapname{#3}}\\
      {\footnotesize \mapname{#1}; $|A|$$=$#2}\\
      \includegraphics[width=1.0\linewidth]{fig/raw/demo_#1}
    \end{minipage}
  }
  %
  \begin{figure}[ht!]
    \centering
    \begin{tabular}{ccc}
      \figcol{random-32-32-20}{409}{random}&
      \figcol{empty-48-48}{1000}{empty}&
      \figcol{ht_chantry}{1000}{chantry}
    \end{tabular}
    %
    \caption{maps}
    \label{fig:maps}
  \end{figure}
}

